GUTS: Generalized Uncertainty-Aware Thompson Sampling for Multi-Agent Active Search

Robotic solutions for quick disaster response are essential to ensure minimal loss of life, especially when the search area is too dangerous or too vast for human rescuers. We model this problem as an asynchronous multi-agent active-search task where each robot aims to efficiently seek objects of interest (OOIs) in an unknown environment. This formulation addresses the requirement that search missions should focus on quick recovery of OOIs rather than full coverage of the search region. Previous approaches fail to accurately model sensing uncertainty, account for occlusions due to foliage or terrain, or consider the requirement for heterogeneous search teams and robustness to hardware and communication failures. We present the Generalized Uncertainty-aware Thompson Sampling (GUTS) algorithm, which addresses these issues and is suitable for deployment on heterogeneous multi-robot systems for active search in large unstructured environments. We show through simulation experiments that GUTS consistently outperforms existing methods such as parallelized Thompson Sampling and exhaustive search, recovering all OOIs in 80% of all runs. In contrast, existing approaches recover all OOIs in less than 40% of all runs. We conduct field tests using our multi-robot system in an unstructured environment with a search area of approximately 75,000 sq. m. Our system demonstrates robustness to various failure modes, achieving full recovery of OOIs (where feasible) in every field run, and significantly outperforming our baseline.

==> nats.tex <==
\section{Noise-Aware Thompson Sampling}
\label{section:nats}

This section presents a brief overview of Noise-aware Thompson Sampling \cite{c1}. Each robot $j$ asynchronously estimates the posterior distribution over OOI locations based on its partial dataset $D_t^j$. During the action selection stage, each robot generates a sample from this posterior and optimizes a reward function for this sampled set of OOI locations. We describe both steps in more detail below.



% \begin{algorithm}
% \caption{(G)NATS Algorithm}
% \label{alg:nats}
% \begin{algorithmic}
% \State \textbf{Assume: }Sensing model (\ref{eqn:sensingmodel}), sparse signal $\betav$, $J$ agents
% \State \textbf{Set: }$\Dv^j_0 \gets \emptyset \enskip \forall j \in \{1,...,J\},\enskip \gamma_m = 1 \enskip \forall m \in \{1,...,M\}$
% \For{$t=1,....,T$}\\
% \quad Wait for an agent to finish; for the free agent j:\\ 
% \quad  Sample $\tilde{\betav} \sim p(\betav|\Dv^j_t, \Gammav)=\mathcal{N}(\muv, \Vv)$ from (\ref{eqn:posteriorbreakdown})
% \qquad\If{NATS} \\\qquad  $\Xv_t = argmax_{\tilde{\Xv}}\Rc(\betav^*, \Dv^j_t,\tilde{\Xv})$ from (\ref{eqn: reward_orig}) \Else\\ \qquad  $\Xv_t = argmax_{\tilde{\Xv}}\Rc(\betav^*, \Dv^j_t,\tilde{\Xv})$ from (\ref{eqn:reward_simple}) in GNATS
% \EndIf\\
% % \quad  Observe $\yv$ and $\Xv$ en route to $\Xv_t$\\
%  \quad  Observe $\yv_t$ given action $\Xv_t$ (trajectory in GNATS)\\
%  \quad  Update $\Dv^j_{t+1}=\Dv^j_t \cup (\Xv_t, \yv_t) $
% \qquad  \If{NATS} Share $\Dv^j_{t+1}$ \Else\\ \qquad Share $(\Xv_t, \yv_t)$ in GNATS
% \EndIf\\
%  \quad  Estimate $\Gammav = diag([\gamma_1,...,\gamma_M])$ using (\ref{eqn:gamma})
% \EndFor
% \end{algorithmic}
% \end{algorithm}


\subsection{Calculating Posterior}

Each robot assumes a zero-mean gaussian prior per entry of the vector $\betav$ s.t. $p_0(\beta_m)=\mathcal{N}(0,\gamma_m)$. The variances $\Gammav = diag([\gamma_1 ...\gamma_M])$ are hidden variables which are estimated using data. We follow \cite{sbl}, \cite{inverse_gamma} and use a conjugate inverse gamma prior on $\gamma_m$ to enforce sparsity s.t. $p(\gamma_m)=IG(a_m,b_m) = \frac{b_m^{a_m}}{\Gamma(a_m)}\gamma_m^{(-a_m-1)}e^{-(b_m/\gamma_m)}\: \forall \: m \in \{1...M\}$. We estimate the posterior distribution on $\beta$ given data $D_t^j$ for robot $j$ using EM.

We can write analytic expressions for the E-step (estimating $p(\beta|D_t^j,\Gamma) = N(\mu, V)$) and M-step (computing $\max_{\Gamma} p(D_t^j| \beta,\Gamma)$) respectively:
\begin{equation}
\label{eqn:e_step}
    V = (\Gamma^{-1}+X^T \Sigma X)^{-1}; \mu = VX^T\Sigma y
\end{equation}
\vspace{-0.5cm}
\begin{equation}
\label{eqn:m_step}
    \gamma_m = ([\Vv]_{mm} + [\muv]^2_m + 2b_m)/(1+ 2a_m)
\end{equation}

Each robot estimates $N(\beta |D_t^j) = N(\mu,V)$ on-board using it's partial dataset $D_t^j$. We drop the index $j$ from equations \eqref{eqn:e_step} and \eqref{eqn:m_step} for clarity. We set the values of $a_m=0.1$ and $b_m=1$ as these were found to be effective in \cite{c1}. Finally, agent $j$ samples from the posterior $\tilde{\betav} \sim p(\betav|\Dv^j_t)$.

\subsection{Choosing Next Sensing Action}
Each robot chooses the next sensing action $\Xv_{t+1}$ by assuming that the sampled set of OOI locations $\tilde{\betav}$ is correct. Specifically, let $\hat{\betav} (\Dv^j_t \cup (\Xv_{t+1}, \yv_{t+1}))$ be our expected estimate of the parameter $\beta$ using all available measurements $\Dv^j_t$ and the next candidate measurement $(\Xv_{t+1}, \yv_{t+1})$. Then the reward function to evaluate each possible sensing action is defined as:
\begin{equation}
    \label{eqn:reward_orig}
    \Rc(\tilde{\betav}, \Dv^j_t, \Xv_{t+1}) = -\mathbb{E}_{\yv|\Xv_{t+1},\tilde{\betav}}[||\tilde{\betav} - \hat{\betav} (\Dv^j_t \cup (\Xv_{t+1}, \yv_{t+1}))||^2_2]
\end{equation}

The reward function is stochastic due to the sampling of $\tilde{\beta}$ and this ensures that the search actions selected by the robots are diverse. 
